Optimizing Feature Set for Click-Through Rate Prediction

Click-through prediction (CTR) models transform features into latent vectors and enumerate possible feature interactions to improve performance based on the input feature set. Therefore, when selecting an optimal feature set, we should consider the influence of both feature and its interaction. However, most previous works focus on either feature field selection or only select feature interaction based on the fixed feature set to produce the feature set. The former restricts search space to the feature field, which is too coarse to determine subtle features. They also do not filter useless feature interactions, leading to higher computation costs and degraded model performance. The latter identifies useful feature interaction from all available features, resulting in many redundant features in the feature set. In this paper, we propose a novel method named OptFS to address these problems. To unify the selection of feature and its interaction, we decompose the selection of each feature interaction into the selection of two correlated features. Such a decomposition makes the model end-to-end trainable given various feature interaction operations. By adopting feature-level search space, we set a learnable gate to determine whether each feature should be within the feature set. Because of the large-scale search space, we develop a learning-by-continuation training scheme to learn such gates. Hence, OptFS generates the feature set only containing features which improve the final prediction results. Experimentally, we evaluate OptFS on three public datasets, demonstrating OptFS can optimize feature sets which enhance the model performance and further reduce both the storage and computational cost.

==> section/introduction_old.tex <==
\section{Introduction}

Click-through rate prediction has been a crucial task in real world commercial recommender systems and online advertising system. It aims to predict the probability of a certain user clicking a recommended item (e.g. movie, advertisement) ~\cite{DeepFM,IPNN,FM,DCN}. The typical CTR input consist of many categorical features. We term the values of these categorical features as feature values, which are organized as feature fields. For example, a feature field \textit{gender} contains three feature values, \textit{male}, \textit{female} and \textit{unknown}. General CTR prediction model first maps all its input features into real-valued dense vectors. Then these vectors fed into feature interaction layer, such as factorization machine ~\cite{FM}, cross network ~\cite{DCN}. The final classifier aggregates these representation vector to make the prediction.

In the general CTR predictive model, the feature selection problem is an important problem that could significantly influence the model performance and run-time inference. The number of features could increase up to millions on web-scale applications. This leads to a large number of embeddings, which contributes to the primary memory bottleneck within both training and inference ~\cite{sfctr}. However, the redundant embedding not only necessitates additional memory cost but is also detrimental to the model performance ~\cite{AutoField,AdaFS,LPFS}. Therefore, it is highly desirable to conduct feature selection in deep CTR prediction.

Selecting an optimal set of features in deep CTR domain should considers several aspects. 
First, the selection of informative features remains an important problem. An feature subset containing the model relevant features to achieve the best performance, remains to be further explored~\cite{RLReview,Elements_SL}. 
Second, the influence of feature selection over feature interaction needs to be considered during the process. The feature interaction indicating the co-existence of different features in one data sample. This problem is especially important and unique for CTR domain as the feature interactions trends to be explicitly modelled in current deep CTR prediction models~\cite{DeepFM,DCN,IPNN}.
Third, a lightweight algorithm should be proposed to efficiently obtain the optimal features under the consideration of previous points.  

However, the majority of previous works have their flaws respectively. 
Hand-crafted feature selection by human expert is usually adopted in traditional CTR system, but such methods requires human experts and tends to be hard to generalize. 
Statistical methods like Lasso regularization~\cite{LASSO} only focus on the feature selection itself, ignoring the influence of feature interaction and prediction models.
Automated methods like AutoField ~\cite{AutoField}, AdaFS ~\cite{AdaFS} are heavy-weighted, requiring extra memory to train the model.
% 把OptFS拿成一个特例来说，没法真正减少memory size

Given the limitation of previous work, an lightweight, model-agnostic method is required in deep CTR domain. Inspired by continual learning, we propose an method named OptFS to set optimal features in the deep CTR prediction. 
We summarize our major contributions as follows:
\begin{itemize}[topsep=0pt,noitemsep,nolistsep,leftmargin=*]
    \item We highlight the three aspects need to be considered for an optimal feature selection methods in deep CTR domains: the influence of feature, the influence of feature interaction and algorithm efficiency. We propose a simple but effective method called OptFS, which improves model performance and reduces memory usage based on these aspects.
    \item The proposed OptFS select the optimal features as an add-on in an end-to-end manner. It performs feature-level selection by continual sparsification.
    \item Extensive experiments are conducted on three public datasets. The experimental results demonstrate the effectiveness and efficiency of the proposed method.
\end{itemize}

We organize the rest of the paper as follows. In Section \ref{sec:method}, we formulate the CTR prediction and feature selection problem and propose a simple but effective method OptFS. Section \ref{sec:experiment} details the experiments. In Section \ref{sec:rw}, we briefly introduce related works. Finally, we conclude this paper in Section \ref{sec:conclusion}.



% Click-through rate prediction has been a crucial task in real world commercial recommender systems and online advertising system. too many features...embedding ...deployment...performance.

% \begin{itemize}
%     \item Feature-level, end-to-end, add-on
% \end{itemize}

% Feature selection should focus on two aspects: 
% \begin{enumerate}
%     \item The selection of feature 
%     \item The influence of feature interaction in terms of feature selection
%     \item The lightweight algorithm to efficiently select feature
% \end{enumerate}



==> section/method_old.tex <==
\section{Method}
\label{sec:method}
In this section, we formulate the CTR prediction model and the feature selection problem.

\subsection{CTR Prediction}
We represent the raw input as:
\begin{equation}
    \mathbf{x} = [\mathbf{x}_{(1)}, \mathbf{x}_{(2)}, \cdots, \mathbf{x}_{(n)}].
\end{equation}

Usually, $\mathbf{x}_{(i)}$ is a one-hot representation, which is very sparse and high-dimensional. For example, the feature field \textit{gender} has three unique feature values, \textit{male},\textit{female}, and \textit{unknown}, then they can be represented by three one-hot vectors $[1,0,0]$,$[0,1,0]$ and $[0,0,1]$, respectively. Before raw feature vectors are fed into the feature interaction layer, we usually employ embedding table to convert them into low dimensional and dense real-value vectors. This can be formulated as $\mathbf{e}_{(i)}=\mathbf{E} \times \mathbf{x}_{(i)}, 1 \le i \le n$, where $\mathbf{E}\in\mathbb{R}^{|f|\times D}$ is the embedding table, $|f|$ is the number of feature values and $D$ is the size of embedding. Then embeddings are stacked together as a embedding vector $\mathbf{e} = [\mathbf{e}_{(1)}, \mathbf{e}_{(2)}, \cdots, \mathbf{e}_{(n)}]$.

Following learnable embedding table, the feature interaction layer will be performed based on $\mathbf{e}$ in mainstream CTR models. There are several types of feature interaction in previous study, e.g. inner product~\cite{DeepFM}. As discussed in previous work~\cite{AutoPI}, feature interaction can be defined as based on embeddings:
\begin{equation}
    \mathbf{v}^p = o^{(p-1)}(o^{(p-2)}(\cdots(o^{(1)}(\mathbf{e}))\cdots)),
    \label{eq:interaction}
\end{equation}
where $o$ can be a single layer perceptron or cross layer\cite{DCN}. The feature interaction can be aggregated together:
\begin{equation}
    \hat{y} = \sigma(\mathbf{w}^T(\mathbf{v}^{(1)}\oplus\mathbf{v}^{(2)}\oplus\cdots\oplus\mathbf{v}^{(m)})+b) = \mathcal{F}(\mathbf{E} \times \mathbf{x}|\mathbf{W}),
    \label{eq:aggregation}
\end{equation}
where symbol $\oplus$ denotes the concatenation operation, $\mathbf{v}^{(k)}$ is the output of feature interaction, and $\mathbf{W}$ is network parameters except for embedding table. The cross entropy loss (i.e. log-loss) is adopted for training the model:
\begin{equation}
\label{eq:logloss}
    \text{CE} (y,\hat{y}) = y\log(\hat{y}) + (1-y)\log(1-\hat{y}).
\end{equation}
We summarize the final CTR prediction problem as follows:
\begin{equation}
\label{eq:summarize}
    \min_{\mathbf{E}, \mathbf{W}} \ \mathcal{L}_{\text{CE}}(\mathcal{D}|\{\mathbf{E}, \mathbf{W}\}) = -\frac{1}{ |\mathcal{D}|} \sum_{(\mathbf{x}, y)\in\mathcal{D}} \text{CE}(y, \mathcal{F}(\mathbf{E} \times \mathbf{x}|\mathbf{W})).
\end{equation}
where $y$ is the ground truth of user clicks, $\mathcal{D}$ is the training dataset. 

\subsection{Optimal Feature Selection}

Originally, all feature are fed into CTR models, which neither efficient nor effective~\cite{AutoField,LPFS,AdaFS}. An optimal feature selection algorithm should consider the following aspects:

\begin{myDef}
\label{def:a1}
\emph{Feature Selection}: The optimal feature selection algorithm table should only map informative feature values to embeddings. Feature value $\mathbf{x}_i$ is considered informative if the performance of the model is degraded when masking its corresponding embedding $\mathbf{e}_i$. Otherwise, it is deemed to be redundant. 
\end{myDef}

\begin{myDef}
\label{def:a2}
\emph{Feature Interaction Selection}: The optimal feature selection algorithm should consider the influence of feature interaction selection.
\end{myDef}

\begin{myDef}
\label{def:a3}
\emph{Algorithm Efficiency}: The optimal feature selection algorithm should be light-weighted and end-to-end trainable.
\end{myDef}

\subsection{OptFS}
\label{sec:optfs}

\subsubsection{Feature Selection}
To consider the three aspects regarding optimal feature subset, we propose the OptFS method as an light-weight, model agnostic approach to efficiently obtain the suitable feature subset given different models and datasets. The feature selection can be formulated as assigning a binary mask $\mathbf{m}_j\in\{0,1\}$ for each feature embedding $\mathbf{e}_j$. Hence, for feature field $i$, suppose the corresponding feature values is $\mathbf{x}_j$, then its feature embeddings can be formulated as: 
\begin{equation}
    \mathbf{e}_{(i)} = \mathbf{m}_j \odot \mathbf{e}_j = \mathbf{m}_j \odot (\mathbf{E} \times \mathbf{x}_j).
\end{equation}

Then, these embeddings are stacked together as a feature-selected embedding vector $\mathbf{e} = [\mathbf{e}_{(1)}, \mathbf{e}_{(2)}, \cdots, \mathbf{e}_{(n)}]$. The final prediction can be formulated as:
\begin{equation}
    \hat{y} = \mathcal{F}(\mathbf{m} \odot \mathbf{E} \times \mathbf{x}|\mathbf{W}) = \mathcal{F}(\mathbf{E}^{m} \times \mathbf{x}|\mathbf{W}),
\end{equation}
where $\mathbf{m}\in\{0,1\}^{|f|}$ refers to mask vectors indicating whether certain feature is selected or not, $\mathbf{E}^m = \mathbf{m} \odot \mathbf{E}$ indicates the feature-selected embedding tables.

\subsubsection{Feature Interaction Selection}

Feature interaction selection

\subsubsection{Continual Sparsification}
To conduct feature selection with feature-level granularity, we introduce a continual mask $\mathbf{m}_c\in\mathbb{R}^{|f|}$. During the training time, we introduce the a exponentially-increased temperature value $\tau$ to approximate $L_0$ normalization. The actual mask is computed as:
\begin{equation}
    \mathbf{m} = \frac{\sigma(\mathbf{m}_c \times \tau)}{\sigma(\mathbf{m}_c^{(0)})},
\end{equation}
where $\mathbf{m}_c^{(0)}$ is the initial value of the continual mask $\mathbf{m}_c$, $\sigma$ is the sigmoid function $\sigma(x) = \frac{1}{1+e^{-x}}$ applied element-wise. Hence, the finally training objective becomes:
\begin{equation}
    \min_{\mathbf{m}_c, \mathbf{E}, \mathbf{W}} \ \mathcal{L}_{\text{CE}}(\mathcal{D}|\{\mathbf{m} \odot \mathbf{E}, \mathbf{W}\}) + \lambda \lVert \mathbf{m}_c \rVert_1,
\end{equation}
where $\lambda$ is the regularization term, $\lVert \cdot \rVert_1$ indicates the $L_1$ norm.

\subsubsection{Rewinding}
After 


\subsection{Method Discussion}
\label{sec:summary}

Table \ref{Table:summary} performs a comprehensive comparison of our approach with others that conduct feature selection. As we can observe, AutoField~\cite{AutoField} and LPFS~\cite{LPFS} conduct field-level feature selection with different approaches. However, the granularity of field-level methods is rather coarse, leading to sub-optimal performance and efficiency. AutoField~\cite{AutoField} and AdaFS~\cite{AdaFS} using bi-level optimization to conduct search for different feature subsets with different granularity. But bi-level optimization requires extra memory during training time, making them sub-optimal for large-scale online system. On the other hand, our proposed method OptFS conduct feature-level subsets via pruning methods the sample with small amount of extra run-time memory, which is caused by the mask vector $\mathbf{m}$.

\begin{table*}[htbp]
\renewcommand\arraystretch{0.9}
\centering
\caption{Comparison of Deep Learning-based Feature Selection Approaches.}
\vspace{-5pt}
\begin{tabular}{c|c|c|c|c|c|c} \hline    
Approach & Granularity & Optimization & Run-time Memory & Pretraining & Retraining & Model Size Reduction \\ \hline
AutoField~\cite{AutoField} & Field   & Bi-lvl Optim        & $2$ & \XSolidBrush & \Checkmark   & \Checkmark    \\ \hline
LPFS~\cite{LPFS}           & Field   & Smoothed $L_0$ norm & $1$ & \XSolidBrush & \XSolidBrush & \Checkmark    \\ \hline
AdaFS~\cite{AdaFS}         & Sample  & Bi-lvl Optim        & $2$ & \Checkmark   & \XSolidBrush & \XSolidBrush  \\ \hline
OptFS                      & Feature & Pruning             & ${1+\frac{1}{D}}$ & \XSolidBrush & \XSolidBrush & \Checkmark    \\ \hline
\end{tabular}
\label{Table:summary}
\end{table*}




